Collaborative Distillation for Top-N Recommendation

Knowledge distillation (KD) is a well-known method to reduce inference latency by compressing a cumbersome teacher model to a small student model. Despite the success of KD in the classification task, applying KD to recommender models is challenging due to the sparsity of positive feedback, the ambiguity of missing feedback, and the ranking problem associated with the top-N recommendation. To address the issues, we propose a new KD model for the collaborative filtering approach, namely collaborative distillation (CD). Specifically, (1) we reformulate a loss function to deal with the ambiguity of missing feedback. (2) We exploit probabilistic rank-aware sampling for the top-N recommendation. (3) To train the proposed model effectively, we develop two training strategies for the student model, called the teacher- and the student-guided training methods, selecting the most useful feedback from the teacher model. Via experimental results, we demonstrate that the proposed model outperforms the state-of-the-art method by 2.7-33.2% and 2.7-29.1% in hit rate (HR) and normalized discounted cumulative gain (NDCG), respectively. Moreover, the proposed model achieves the performance comparable to the teacher model.

==> Figures/exp_fig1.tex <==
\begin{figure*}[t]
\centering
\begin{tabular}{cccc}
\includegraphics[width=0.23\textwidth]{Figures/figure3_1.png} &
\includegraphics[width=0.23\textwidth]{Figures/figure3_2.png} &
\includegraphics[width=0.23\textwidth]{Figures/figure3_3.png} &
\includegraphics[width=0.23\textwidth]{Figures/figure3_4.png} \\
(a) AMusic (CDAE) & (b) AMusic (Caser) & (c) Yelp (CDAE) & (d) Yelp (Caser) \\
\end{tabular}
\caption{NDCG@50 across three different model sizes. XS, S, and M indicate 10\%, 20\%, 30\% of the size of teacher model, respectively. }\label{fig:modelvseffectiveness}
\end{figure*}


\begin{figure*}[t]
\centering
\begin{tabular}{cccc}
\includegraphics[width=0.23\textwidth]{Figures/figure4_1.png} &
\includegraphics[width=0.23\textwidth]{Figures/figure4_2.png} &
\includegraphics[width=0.23\textwidth]{Figures/figure4_3.png} &
\includegraphics[width=0.23\textwidth]{Figures/figure4_4.png} \\
(a) AMusic (CDAE) & (b) AMusic (Caser) & (c) Yelp (CDAE) & (d) Yelp (Caser) \\
\end{tabular}
\caption{Online inference latency vs. model size. In both datasets, the inference latency is greatly reduced by decreasing the model parameters.}\label{fig:modelvsinference}
\end{figure*}


\begin{figure*}[t]
\centering
\begin{tabular}{cccc}
\includegraphics[width=0.23\textwidth]{Figures/figure5_1.png} &
\includegraphics[width=0.23\textwidth]{Figures/figure5_2.png} &
\includegraphics[width=0.23\textwidth]{Figures/figure5_3.png} &
\includegraphics[width=0.23\textwidth]{Figures/figure5_4.png} \\
(a) AMusic (CDAE) & (b) AMusic (Caser) & (c) Yelp (CDAE) & (d) Yelp (Caser) \\
\end{tabular}
\caption{NDCG@50 vs. the number of epochs. As the epoch increases, the performance gap between our model and teacher model is reduced.  }\label{fig:iterations}
%\vskip -0.2in
\end{figure*}

==> Figures/exp_fig2.tex <==

\begin{figure}[t]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.23\textwidth]{Figures/figure6_1.png} &
\includegraphics[width=0.23\textwidth]{Figures/figure6_2.png} \\
(a) AMusic (CD-SG) & (b) Yelp (CD-SG) \\
\end{tabular}
\caption{NDCG@50 vs. KD parameter $\lambda$ (CDAE). In both datasets, our model is the best in $\lambda = 0.1$. }\label{fig:kdparameter}
\end{figure}


\begin{figure}[t]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.23\textwidth]{Figures/figure7_1.png} &
\includegraphics[width=0.23\textwidth]{Figures/figure7_2.png} \\
(a) AMusic (CD-SG) & (b) Yelp (CD-SG) \\
\end{tabular}
\caption{NDCG@50 vs. sampling ratio $\delta$ (CDAE).  In AMusic and Yelp, our model is the best in $\delta = 0.5$.}\label{fig:samplingratio}
\vskip -0.2in
\end{figure}


==> Figures/exp_table1.tex <==
\begin{table*}[t]
\caption{Performance comparison of each model in four benchmark datasets.}\label{tab:com1}
\begin{center}
\begin{tabular}{p{1cm}p{1.1cm}p{1.1cm}p{1.5cm}p{1.1cm}p{1.5cm}p{1.1cm}p{1.5cm}p{1.1cm}p{1.5cm}}
\toprule
\multicolumn{2}{c}{Models} & \multicolumn{2}{c}{AMusic} & \multicolumn{2}{c}{ML100K} & \multicolumn{2}{c}{Yelp} & \multicolumn{2}{c}{Gowalla}\\
 &  & HR@50 & NDCG@50 & HR@50 & NDCG@50 & HR@50 & NDCG@50 & HR@50 & NDCG@50  \\
\hline
\multirow{7}{*}{CDAE}
& Teacher & 0.1727 & 0.0547 & 0.3917 & 0.1288 &0.1150 & 0.0340 & 0.3057 & 0.1269 \\
& Student & 0.1217 & 0.0370 & 0.3565 & 0.1107 &0.0956 & 0.0278 & 0.2632 & 0.1088 \\
& RD & 0.1275 & 0.0402 & 0.3578 & 0.1112 & 0.0949 & 0.0272 & 0.2638 & 0.1092 \\
& RD-Rank & 0.1238 & 0.0366 & 0.3580 & 0.1110 & 0.0915 & 0.0258 & 0.2602 & 0.1034 \\
& CD-Base & 0.1613 & 0.0498 & 0.3707 & 0.1124 & 0.1042 & 0.0304 & 0.2613 & 0.1093 \\
& CD-TG & \text{0.1653} & \text{0.0513} & \textbf{0.3805} & \text{0.1175} &\text{0.1060} & \text{0.0309} & \text{0.2682} & \text{0.1113} \\
& CD-SG & \textbf{0.1681} & \textbf{0.0519} & \text{0.3741} & \textbf{0.1182} & \textbf{0.1067} & \textbf{0.0313} & \textbf{0.2710} & \textbf{0.1122}\\
\cline{2-10}
& Gain (\%) & 31.84 & 29.1 & 6.34 & 6.29 & 12.43 & 15.07 & 2.72 & 2.74\\
\hline
\multirow{7}{*}{Caser}
& Teacher & 0.1366 & 0.0392 & 0.3145 & 0.0868 & 0.0947 & 0.0266 & 0.3005 & 0.1109 \\
& Student & 0.0919 & 0.0276 & 0.2717 & 0.0730 & 0.0789 & 0.0220 & 0.2033 & 0.0768 \\
& RD & 0.0936 & 0.0276 & 0.2732 & 0.0758 & 0.0814 & 0.0230 & 0.2358 & 0.0877 \\
& RD-Rank & 0.0909 & 0.0271 & 0.2787 & 0.0774 & 0.0813 & 0.0232 & 0.2362 & 0.0880\\
& CD-Base & \textbf{0.1211} & \textbf{0.0355} & 0.3147 & 0.0872 & 0.0874 & 0.0244 & 0.2557 & \textbf{0.0943} \\
& CD-TG & 0.1138 & 0.0337 & \textbf{0.3203} & \text{0.0879} & 0.0899 & 0.0249 & \text{0.2525} & \text{0.0904} \\
& CD-SG & \text{0.1188} & \text{0.0352} & 0.3196 & \textbf{0.0891} & \textbf{0.0965} & \textbf{0.0269} & \textbf{0.2570} & 0.0925 \\
\cline{2-10}
& Gain (\%) & 29.38 & 28.62 & 17.24 & 17.54 & 18.55 & 16.95 & 8.99 & 7.52\\
\hline
\bottomrule
\end{tabular}
\end{center}
\vskip -0.2in
\end{table*}

%Gain indicates how high the accuracy of the proposed model is over RD. The difference between RD and proposed model is statistically significant based on a one-tail t-test, with 95\% confidence.

==> Figures/fig1.tex <==
\begin{figure}
%\includegraphics[width=0.7\textwidth]{Figures/RD.pdf}
\includegraphics[width=\linewidth]{Figures/figure1.png}
\caption{Illustration of \emph{rank distillation} (RD)~\cite{TangW18b}. The teacher model transfers manipulated top-K items as the distilled knowledge to the student model.}\label{fig:RD}
\vskip -0.2in
\end{figure}


==> Figures/fig2.tex <==
\begin{figure}
\includegraphics[width=\linewidth]{Figures/figure2.png}
\caption{Illustration of \emph{collaborative distillation} (CD).  The teacher model transfers soft targets to student model. The probabilistic rank-aware sampling is adopted for placing more weights on high-ranked items.}\label{fig:CD}
\vskip -0.2in
\end{figure}



==> Figures/fig_SG.tex <==
\begin{figure}
\includegraphics[width=\linewidth]{Figures/figure_SG.png}
\caption{Illustration of student-guided training. The student-guided training dynamically determines the teacher's soft target during student's inference.}\label{fig:SG}
%\vskip -0.2in
\end{figure}
